Learning an Adaptive Forwarding Strategy for Mobile Wireless Networks: Resource Usage vs. Latency

Designing effective routing strategies for mobile wireless networks is challenging due to the need to seamlessly adapt routing behavior to spatially diverse and temporally changing network conditions. In this work, we use deep reinforcement learning (DeepRL) to learn a scalable and generalizable single-copy routing strategy for such networks. We make the following contributions: i) we design a reward function that enables the DeepRL agent to explicitly trade-off competing network goals, such as minimizing delay vs. the number of transmissions per packet; ii) we propose a novel set of relational neighborhood, path, and context features to characterize mobile wireless networks and model device mobility independently of a specific network topology; and iii) we use a flexible training approach that allows us to combine data from all packets and devices into a single offline centralized training set to train a single DeepRL agent. To evaluate generalizeability and scalability, we train our DeepRL agent on one mobile network scenario and then test it on other mobile scenarios, varying the number of devices and transmission ranges. Our results show our learned single-copy routing strategy outperforms all other strategies in terms of delay except for the optimal strategy, even on scenarios on which the DeepRL agent was not trained.

==> bing-command.tex <==

% \usepackage{epsfig}
% \usepackage{algorithm}
% \usepackage{algorithmic}
%\usepackage{algpseudocode}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

% \newcommand{\mysection}[1]{\vspace{-.03in}\section{#1}\vspace{-.00in}}
% \newcommand{\mysubsection}[1]{\vspace{-.05in}\subsection{#1}\vspace{-.01in}}
% \newcommand{\mysubsubsection}[1]{\vspace{-.05in}\subsubsection{#1}\vspace{-.00in}}

% \newcommand{\remove}[1]{}

\newtheorem{goal}{Goal}
\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}[section]
\newtheorem{corollary}{Corollary}

\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{Lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.28\textwidth}
 \epsffile{\Figdir#1}
 \vspace{-2ex}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.22\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.24\textwidth}
 \epsffile{\Figdir#1}
 \vspace{-2ex}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\bigdubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.98\textwidth}
        \setlength{\epsfysize}{0.90\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace{-0.05in}
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.98\textwidth}
        \setlength{\epsfysize}{0.90\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}


\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
    \vspace{-2ex}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.45\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
    \vspace{-2ex}
} \caption{#5}\label{fig:#6}
\end{figure}
}

\iffalse
\newcommand{\tyfourfigsingle}[10]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#5}
       \newline{\small (a) #6}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#7}
       \newline{\small (b) #8}
      \end{center}
    \end{minipage}
} \caption{#9}\label{fig:#10}
\end{figure}
}
\fi

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.90\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.90\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        %\setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.70\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.70\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.70\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
%\vspace*{-0.2in}
\end{figure*}
}

% a triplefig for wider figures
\newcommand{\triplefigwide}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        %\setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.70\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.70\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.70\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
    \vspace{-2ex}
} \caption{#7}\label{fig:#8}
%\hrule
%\vspace*{-0.2in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> mobility-long.tex <==
\subsubsection{Device Mobility}
\label{sec:connectivity}

We use BonnMotion \cite{aschenbruck2010bonnmotion} to generate 
mobility traces for devices moving under the {\em steady-state random waypoint (RWP) mobility model} \cite{navidi2004stationary,navidi2004improving,le2005perfect} and the {\em original Gauss-Markov (GM) mobility model} \cite{Liang99:Gauss-Markov}. 
For both mobility models, BonnMotion generates a mobility trace as a sequence of waypoints for each device. For example, device $v$'s mobility is a sequence of waypoint tuples: $(t_0^v, x_0^v, y_0^v)$, $(t_1^v, x_1^v, y_1^v),..., (t_i^v, x_i^v, y_i^v)...$, where device $v$ changes its waypoint at time $t_1^v, t_2^v, ...$, and during during $[t_i^v, t_{i+1}^v]$, device $v$ moves from location $(x_i^v,y_u^v)$ to location $(x_{i+1}^v,y_{i+1}^v)$ at a constant speed. 
% Because these waypoints occur and are thus recorded at arbitrary points in time, we must convert the tuples to match our simulation timesteps, where each timestep corresponds to one second. 
Because the times when waypoint changes are decided by the mobility model, however, and  these times do not coincide with the timesteps in our simulation, we calculate the locations of each device at each timestep as follows, where each timestep corresponds to one second. 
The location of device $v$ at each timestep $t$ is calculated by first finding the time interval $[t_k^v, t_{k+1}^v]$ in which $t$ falls in, and then calculating the location at time $t$ via a linear interpolation of $(x_k^v,y_k^v)$, $v$'s location at $t_k$, and $(x_{k+1}^v, y_{k+1}^v)$, $v$'s location at $t_{k+1}$. 


\begin{figure}[t]
\centerline{\hbox{
    \subfigure[Random waypoint mobility]
    {\includegraphics[width=1.15in]{plots-stats/stats_variable__data-mob-features-directtx-steadystaterandomwaypoint-test_NODE_DEGREE.png}
    \hspace{-0.05in}
    \includegraphics[width=1.15in]{plots-stats/stats_variable__data-mob-features-directtx-steadystaterandomwaypoint-test_PROBABILITY_PATH_EXISTS.png}
    \hspace{-0.05in}
    \includegraphics[width=1.25in]{plots-stats/stats_variable__data-mob-features-directtx-steadystaterandomwaypoint-test_AVG_INTERMEETING_TIME.png}
    \hspace{-0.05in}
    \includegraphics[width=1.15in]{plots-stats/stats_variable__data-mob-features-directtx-steadystaterandomwaypoint-test_AVG_MEETING_DURATION.png}}
    }}
    \vspace{-0.05in}
    \centerline{\hbox{
    \subfigure[Gauss-Markov mobility.]
    {\includegraphics[width=1.15in]{plots-stats/stats_variable__data-mob-metrics-directtx-origgaussmarkov_NODE_DEGREE.png}
    \hspace{-0.05in}
    \includegraphics[width=1.15in]{plots-stats/stats_variable__data-mob-metrics-directtx-origgaussmarkov_PROBABILITY_PATH_EXISTS.png}
    \hspace{-0.05in}
    \includegraphics[width=1.25in]{plots-stats/stats_variable__data-mob-metrics-directtx-origgaussmarkov_AVG_INTERMEETING_TIME.png}
    \hspace{-0.05in}
    \includegraphics[width=1.15in]{plots-stats/stats_variable__data-mob-metrics-directtx-origgaussmarkov_AVG_MEETING_DURATION.png}}
    }}
\caption{{\small Quantifying the connectivity of the network scenarios considered during testing. }}
% In (a) and (b) we show that the different numbers of devices and transmission ranges we consider in our simulations encompass the continuum from disconnected to well-connected networks. In (c) and (d), we show the inter-meeting time $T_{v,d}$ and meeting duration $M_{v,d}$ of Section \ref{sec:path-features}: these metrics are computed online between each possible pair of devices, and so are independent of the number of devices.}}
\label{fig:rl-connectivity}
\end{figure}

\color{red}
The RWP mobility model picks, for each device, a random point on the simulation area, a random speed is picked. The device then travels to that point at the chosen speed. Once it arrives, the device pauses for a randomly chosen pause time, and then repeats the process until the simulation ends. 
The Steady-State RWP  picks initial device positions, speeds, and pause times according to the steady-state distributions of the RWP model, so that no time is required at the beginning of the simulation to let the distributions of position and speed settle. 

GM model is a temporally dependent mobility model. Under GM model, each device is assigned an initial speed and direction. Subsequently, at fixed intervals of time, each device's speed and direction is updated. More specifically, the speed (and direction) of a device at the $n$-th interval, denoted as $s_n$ (and $d_n$) is calculated as follows:
\begin{eqnarray*}
s_n &=& \alpha s_{n-1} + (1-\alpha)\bar{s} + \sqrt{(1-\alpha^2)s_{x_{n-1}}} \\
d_n &=& \alpha d_{n-1} + (1-\alpha)\bar{d} + \sqrt{(1-\alpha^2)d_{x_{n-1}}}\end{eqnarray*}

where $ 0 \leq \alpha \leq 1 $ is a parameter used to vary the temporal dependency, $\bar{s}$ and $\bar{d}$ are the mean speed and direction, and $s_{x_{n-1}}$ and $d_{x_{n-1}}$ are random variables from a Gaussian distribution.


RWP mobility model gives rise to a different spatial distribution of devices in the network compared with GM. Under RWP, devices are more concentrated near the center of the simulation region~\cite{navidi2004stationary}; whereas under GM model, devices are evenly distributed in the simulation region. As a result, we observe that a higher node degree (and probability of path exists, ...) under RWP compared to GW. 
Importance of steady-state
More clustered in center
GM ...
More evenly distributed ...

\color{black}

For training, we use RWP and GM mobility traces of $N_{train}=25$  devices moving in a 500m $\times$ 500m area. For RWP traces,  devices move around at an average speed of 3 m/s with a speed delta of 2 m/s and  a transmission range of $X_{train}$=50m. 
\color{red}
For GM traces, devices move around at ..
\color{black}
For testing, we generate separate RWP and GM mobility traces for $N=25, 64, 100$ devices using the same size area and range of speeds, but vary the transmission  range, $X_{test}$ from 30m to 80m to obtain both poorly connected and very well connected mobile scenarios, see Fig.~\ref{fig:rl-connectivity}.

Fig. \ref{fig:rl-connectivity} quantifies the connectivity of the network scenarios we consider in our simulations.
In Figs. \ref{fig:rl-connectivity}(a) and (b) we show that the different numbers of devices and transmission ranges we consider in our simulation experiments encompass the continuum from disconnected to well-connected networks. In Figs. \ref{fig:rl-connectivity}(c) and (d), we show the average inter-meeting time and meeting duration between pairs of devices:
%$T_{v,d}$ and meeting duration $M_{v,d}$ of Section \ref{fig-meeting-trace}:
these metrics are computed online between each possible pair of devices, and so are independent of the number of devices. 
% For additional details about our simulations and extensive simulation results, please see \cite{manfredi2022learning}.

==> one-hop-delay.tex <==
 %%this uses \widehat notation
 
     \item {\em Expected one-hop delay}  from  device $v$ to  device $d$, denoted as $D^{(1)}_{v,d}$, which is the expected delay when $v$ directly transmits the packet to $d$, i.e., in one-hop, without using any intermediate node. 
     %Let $\widehat{T}_{v,d}$  and $\widehat{M}_{v,d}$ denote the estimated average inter-meeting time and meeting duration between $v$ and $d$, respectively. Consider the entire 
     To derive this quantity, consider the time period from when $v$ and $d$ first move out of each other's transmission range until they move into each other's transmission range again. It is $\widehat{T}_{v,d}+\widehat{M}_{v,d}$, where $\widehat{T}_{v,d}$ and $\widehat{M}_{v,d}$ denote the estimated average inter-meeting time and meeting duration between $v$ and $d$, respectively. Therefore, at any point of time $t$, the expected delay for transmitting one packet from $v$ to $d$ is  
    \begin{eqnarray}
    \label{eq:direct-one-hop}
    D^{(1)}_{v,d} = 1 \times \frac{\widehat{M}_{v,d}}{\widehat{T}_{v,d}+\widehat{M}_{v,d}} + \Delta_{v,d} \times \frac{\widehat{T}_{v,d}}{\widehat{T}_{v,d}+\widehat{M}_{v,d}},
    \end{eqnarray}
    where the first term represents the expected delay when the two nodes are already in the transmission range of each other (under such conditions, the latency is one time slot), while the second term represents the expected delay when the two nodes need to meet each other first and then $v$ transfer the packet to $v$, where $\Delta_{v,d}$ is the expected time from an point of time $t$ to when the two nodes meet each other. Following queuing theory \cite{kleinrock:qtheory}, we estimate $\Delta_{v,d}$  as $ \Delta_{v,d} = \widehat{T}_{v,d}/2 + \sigma^2_{v,d}/(2  \widehat{T}_{v,d})$, 
    %$$ \Delta_{v,d} = \frac{\widehat{T}_{v,d}}{2} +\frac{\sigma^2_{v,d}}{2  \widehat{T}_{v,d}  }$$
   where $\sigma^2_{v,d}$ is the estimated variance of this inter-meeting time. We obtain estimate of $\widehat{T}_{v,d}$ and $\widehat{M}_{v,d}$ over time in an online manner, and then use Eq. (\ref{eq:direct-one-hop}) to estimate $D^{(1)}_{v,d}$. 

==> to-add.tex <==

To-add for journal version: 
\begin{itemize}


    Gauss-markov: can tune to have different amounts of memory. Alpha parameter used in next trip to decide how much speed and direction depend on last location?


    Do we ever train on queue lengths of non-zero?  Need to train on more congested scenario, maybe N=25, tx = 30

    Train on N=64, tx=30, tx=50
    Mixed training/Meta
    
    Update overfitting: regularization, dropout, 


    Update rlagent to not use location in timer estimate of distance to neighbor? Rlagent currently uses the utility, so once utility updated other routers will be udpated unless we add a flag to switch 
    
    timer transitivity/state updates: synchronization issues? Delay by one timestep? Add description to paper
    All algorithms will have the same synchronization issues?
    All path features will also have synchronization issue?

    Differentiate timer values by neighbor

    Two neighbors meet, have same timer transitivity value, then how does help as feature? Also have distance to other node with lower timer to destination
    
    \item Feature ablation: with/without distance, with/without timer transitivity, with/without inter-meeting/duration

    Meta learner: train on N=25, tx=30, tx=50, N=64
    Predictability, connectivity features for sparse network
    Predicting future neighbors for sparse network

    When sparse: start making a lot of stay decisions rather than the more random forwarding decisions that seek and focus makes.


    Non-determinstic policy (e.g., random forwarding useful when nework is sparse) then move to policy gradient

    add feature flag: do I trust feature yet or not. 0/1 or average of intermeeting and number of meetings normalized

    When network is sparse, is operating randomly beneficial? Is that what seek-and-focus is doing? So either wait for destination or forward frequently beneficial when long inter-meeting times, unpredictable? And for these models, nodes do eventually meet each other, which is why direct transmission can do well when sparse? This sparse scenario is really multi-copy scenario (for which we first need device decisions)

    % Check normalization value for n=25, tx=30 scenario for timer to make sure 800 is okay to normalize by.

    %  can we use a very simple synthetic mobility trace, e.g., with only 3 nodes, A and B meet at time t1, B and C meet at t2, and A, B and C meet at time t3, to just quickly verify that we got the timing information as expected? Please ignore if this does not make sense.

    % Plot timer vs. distance values, for N=25, tx=30,50
    % As delay between meetings increases, more innacuracy in timer. Include plots in paper

    % Plot evolution of timer value over time? For just one node to another destinations, along with node neighbors (actions under consideration)
    
    % try training on the N=25, tx=30m scenario: if performance is poor here, that might tell us it isn’t just a generalization issue.

    % how different are neighbors in terms of timers, can we plot? how different are distances between neighbors?

    % When two nodes first meet: distance is transmission range. Normalize distance between nodes by this?

    % RWP hist5
    % done    distance,    no timer
    % running no distance, no timer (DELAY OK, BUT HIGH # OF HOPS, PACKET DROPS)
    % running distance,    timer  
    % running no distance, timer  (DELAY LESS OKAY, NOT ALL PACKETS DELIVERED, QUEUE BUILD_UP)
    % running no distance, timer, last inter-meeting, last duration, time-at-node (IMPROVEMENT)

    % TO RUN no distance, timer, time-at-node 
    % TO RUN no distance, timer, last inter-meeting, last duration
    % TO RUN no distance, no timer, last inter-meeting, last duration, time-at-node 

    
    % GM hist5
    % running distance,    no timer
    % running no distance, no timer
    % running distance,    timer
    % running no distance, timer
  
    % done Plot 2d reward/delay plots using test data: 25, 64
    % Plot training results for random waypoint feature ablation
    % Plot training results for gauss markov feature ablation
    % Start testing for random waypoint feature ablation
    % Start testing for gauss markov, feature ablation
    % Start training for Manhattan
 
 
    % Manhattan hist5
    % distance,    no timer
    % no distance, no time
    % distance,    timer
    % no distance, timer
   
    % distance,    no timer
    % no distance, no timer
    % distance,    timer
    % no distance, timer


    \item Gauss-markov, (Manhattan)
    \item Cross-model testing
    \item Reward/history trade-off graph: testing results for this
    \item Euclidean distance replacement
    \item localization without gps: discuss?

    
    \item Hybrid scenario
    \item Intermeeting, meeting duration, average and more recently weighted average
    \item Aggregate inter-contact time vs individual inter-contact time 
    \item Meta-learner with inter-meeting times 
    \item stretch goal: hand-coded packet selection, or discussion of this
    \item estimated distance instead of distance: that wording
    \item seek and focus with distance?
\end{itemize}

Discussion to-add for journal version: 
\begin{itemize}
    \item discussion of mobility models: differences, what they mean for routing, and how they differently distribute nodes in the area.
    \item Doubly emphasize the decentralized aspects of the problem
    \item Euclidean distance: discuss what work assumes location is know.
    \item Need much more extend related work discussion. More discussion in related work clearly explaining deficiencies in existing work. Work is just not comparable, they are maybe not solving the same problem?
    May be useful to talk non-mobile related work on routing/DRL if good papers.
    \item More details about the packet agent and training: include dataframe construction from wowmom paper?
    \item More discussion of how we did normalization and why normalize.
    \item Trying to quantify control overhead
    \item Size of state space/action space
    \item In addition, the structure of the neural network is not elaborated on in the paper, so it would be better if some details about the network (such as structure and training details) are introduced.

    \item As the paper described, there are 5 relational features in total, with many of them having relations with others (for example, the neighborhood feature can be seen as an information compression of device features and path features). It is appreciated if the relations (similarities and differences) among those features can be elaborated in a table, which will be beneficial for the understanding of the construction and the considerations of the relational features. 

    \item Feature ablation in terms of whole classes of features. The necessity of the components of the relational features lacks experimental verification. Due to the complicated construction of the relational features (5 components in total), it is appreciated to verify whether they are all necessary for the agent to perform well, which is currently unshown in the paper.
    \item mark optimal as oracle, change use of optimal to oracle
    
    \item The description of the weighted reward function, which is claimed as a key contribution of this paper, is not clear.
    
    \item What is the state-of-the-art DRL-based packet forwarding scheme for mobile networks? How does the proposed approach perform compared with the state-of-the-art work?

    \item The authors should be more specific in their related work section how their work differs and is similar to other Hierarchical RL works. Given there is no hierarchy of actions, I'm not sure the use of the term is appropriate. The authors only simulate scenarios in which each device has enough bandwidth to transmit all packets (parameter k). 
    \item It is not clear how their approach would perform in bandwidth-limited scenarios and how reward should be tuned for that.

    \item - The authors use experience replay, as "the relational features are device and network independent". However, given devices estimate information about other devices, the same observation could be obtained from two very different states. For example, the source device $v$ is close to device $u$, so gets information from $u$ of timestamped locations. Let's say $u$ saw the goal device $d$ in the past, but after that $d$ could have moved closer or further from $u$, we don't know and it affects the next state. Why is that uncertainty not a problem when using experience replay?
    \item 
    \item What is the total dimensionality of the state? It would be interesting to know
    \item Provide better insights on how operators can interact with the two objectives explored. Right now there is no clear answer to that question other than trial-and-error. If the authors want to frame this problem as a multi-objective problem in the real world, then all the analysis should be framed around better dealing with multiobjectiveness.
    \item It would greatly benefit the paper if the authors can find a set of scenarios in which DRL improves upon both delay and number of hops compared to the other strategies.
\end{itemize}



Future work: 
\begin{itemize}
    \item Delay features: delay + direction: to avoid distance
    \item CQ+-routing: use path estimates as features.
    \item Incorporate uncertainty/confidence, look at CQ-routing related papers for inspiration. Maybe look at weak state routing work
    \item Basic packet selection scheme
    \item Device layer/Packet selection (start with static then mobile)
    \item Multi-copy packets 
    \item Extend the simulations to include more real-world elements (e.g., noise, sudden packet loss, a specific problem as context)

\end{itemize}

